On Area Growth in Sol

Let Sol be the $3$-dimensional solvable Lie group whose underlying space is $\mathbb{R}^3$ and whose left-invariant Riemannian metric is given by $$e^{-2z} dx^2 + e^{2z} dy^2 + dz^2.$$ Building on previous joint work with Matei Coiculescu, which characterizes the cut locus in Sol, we prove that the sphere of radius r in sol has area at most $20 \pi e^r$ provided that r is sufficiently large. This estimate is sharp up to a factor of 10

==> Junk/7iso_old.tex <==
\subsection{Proof of the Embedding Theorem}
\label{embedproof}

In this chapter we prove the Embedding Theorem.
Let $\underline \Lambda_L=
(\underline a_L,\underline b_L)$, as in
\S \ref{diffeq}.  Let $E$ be the Riemannian exponential map
and let $\eta_Z$ be projection into the plane $\Pi_Z$.
We have $\Upsilon_r=\eta_Z \circ E(Y_r^*)$, where
$Y_r^*$ is the relevant component of $Y_r$.

\begin{lemma}
  $\Upsilon_r(L)=\underline \Lambda_L(r)$.
\end{lemma}

\startproof
Recall that $S_r'$ is the set of perfect vectors of length
$r$ contained in the positive sector of $\R^3$.
Let $V \in S_r'$ be a vector such that
$V/\|V\|$ lies in the loop level set of period $L$.  We claim that
$U \in Y_r$ is and only if the flowline associated to $V$ ends in
the plane $\Pi_Z$.   Such a flowline is the initial half
of a symmetric flowline that winds at most twice around
the corresponding loop level set.  The Doubling Lemma then
tells us that
\begin{equation}
\eta_Z \circ E(U)=\underline \Lambda_L(r)=\Upsilon_r(L).
\end{equation}
So, the claim above finishes the proof of the lemma.

Let $T_V$ be the tangent plane to $S_r'$ at $V$.
Let $N_V$ denote the unit outward normal to $T_V$.
Since $V$ is a small vector, Theorem
\ref{main2} tells us that the differential
$dE$ is non-singular at $V$.  (We proved this
explicitly in connection with our
Cut Locus Theorem in [{\bf CS\/}].)  As is
well known, $dE_V(T_V)$ and $dE_V(N_V)$ are
orthogonal.  If
$d(\eta_Z \circ E)$ is singular at $V$, then
$dE_V(T_V)$ contains the vector $(0,0,1)$.

At every tangent plane of Sol, the space of
vectors orthogonal to $(0,0,1)$ is spanned
by the vectors $(1,0,0)$ and $(0,1,0)$.  Hence
$dE_V(N_V)$ is a linear combination of these
vectors.  In particular, the third coordinate
of $dE_V(N_V)$ is $0$.   Note finally that
$dE_V(N_V)$ is the unit tangent vector $\gamma'(r)$ to
the geodesic segment $\gamma$ corresponding to $V$,
at $\gamma(r)$.  But $\gamma'(r)$ lies in the same
left-invariant
vector field as the unit vector at the
end of the flowline associated to $V$.
Hence, this endpoint must have third
coordinate $0$.
\endproof

  We call $\Upsilon_r$ an
  {\it isochronal curve\/} because it
  computes all the solutions to the
  differential equation at the
  fixed time $r$.  Figure 7.1 shows
  part of $\Upsilon_5$.  The blue curves
  are the various curves $\underline \Lambda_L[0,L]$.
        
  \begin{center}
  \resizebox{!}{2in}{\includegraphics{Pix/fig8.eps}}
  \newline
  {\bf Figure 7.1:\/} The $\underline \Lambda_L$ curves and the
  initial part of $\Upsilon_5$.
  \end{center}

  The expression $\Upsilon_r[a,b]$ denotes the
  image of $[a,b]$ under the map $\Upsilon_r$.

\begin{lemma}
  \label{tail}
  The curve $\Upsilon_r[2r,\infty)$ is smooth, regular,
    and embedded.
\end{lemma}

\startproof
The flowline corresponding to the point $\Upsilon_r(t)$  lies
on the loop level set of period $t$ and exists for time $r$.
If $t> 2r$ then the flowline travels less than halfway
around the loop level set.  Thus, the flowline is the
initial half of a small symmetric arc.

Let $S \subset \R^3$ denote the set of vectors corresponding
to small symmetric flowlines. Let $S_L \subset S$ denote
the subset of vectors $V$ such that $V/\|V\|$ lies in the
loop level set in the positive sector having period $L$.
The Riemannian exponential map
$E$ is a diffeomorphism on $S$.  By the Doubling Lemma,
$$\Upsilon_r(2r,\infty)=\frac{1}{2} E(C_r),$$
where $C_r \subset S$ is a curve.  This curve is
embedded because $C_r$ intersects each $C_L$ once
for each $L \in (2r,\infty)$.  Since $E$ is a diffeomorphism
on $S$, we see that $E(C_r)$, and hence
also $\frac{1}{2}E(C_r)$, is embedded.
\endproof




We have already seen that $\Upsilon_r[2r,\infty)$ is
a smooth regular curve.  So, we just have to
analyze $\Upsilon_r[r,2r)$.
  The velocity of
  $\Upsilon_r$ at $L$ is
  $$\bigg(\frac{\partial \underline a_L}{\partial L},\frac{\partial \underline b_L}{\partial L}\bigg)\bigg|_r.$$
    By Equation \ref{Matei3}, this expression equals
    vanishes if and only if $\partial b_L/\partial L(r)=0$.
  So, by the Monotonicity Lemma,
  $\Upsilon[2r,\infty)$ only has one cusp.

      This completes the proof of the Embedding Theorem.


\newpage


  














==> Junk/7old.tex <==
\section{The Vahishing Point}

\subsection{Auxiliary Functions}

The goal of this chapter is to prove the
Monotonicity Lemma.  Our functions depend on the parameter $L$,
which corresponds to the initial conditions of the ODE, and on
the parameter $t$, which is the time parameter for the ODE.
We set $f'=\partial f/\partial t$ and $\dot f = \partial f/\partial L$
We introduce the following $4$ functions:

\begin{equation}
  \label{mainfunctions}
  Z = \dot z, \hskip 15 pt
  X=\dot y/y, \hskip 15 pt
  Y=\dot z/z, \hskip 15 pt
  B=\dot b/b, \hskip 15 pt
\end{equation}
Since $a,b,x,y>0$ these functions respectively  have
the same signs as $\dot z, \dot x, \dot y, \dot b$.

  \begin{center}
  \resizebox{!}{3.1in}{\includegraphics{Pix/fig12.eps}}
  \newline
      {\bf Figure 7.1:\/} Numerical plots
   \end{center}

The top half of
Figure 7.1 shows numerical plots of these functions at $L=8$.
The bounding box in the picture is $[0,8] \times [-1,1]$.
The bottom half shows the plot of the functions at the value $L=16$.
This time we are just showing the right half of the plot.  Notice that
in the interval $[L-1,L]$ the plots line up very nicely.
The black dot in both cases is the point $(t_L,0)$.  One half
of the Monotonicity Lemma establishes that $t_L$ is uniquely
defined.  The second half shows that $t_L$ increases monotonically.
The intuition behind the second half of the result is that
the pictures in $[L-1,L]$ stabilize, so that $t_L=L-s_L$
where $\partial s_L/\partial L$ is approximately $0$ for large $L$.

\subsection{Differentiation Formulas}

Here we give some useful formulas for the
derivatives of the functions above.
\begin{itemize}
\item  $X' =  -Z$
\item  $Y' =  +Z$
\item  $Z'=- 4y^2Y -2z Z.$
\item $B'= \frac{y}{\underline b}(Y - B) - Z.$
\item $Z''=(-2+6z^2)Z$.
\end{itemize}
With some of the formulas we have broken symmetry
and expressed them entirely in terms of $Y,Z,B$.
\newline
\newline
{\bf Representative Derivations:\/}
We will derive two of these identities.  The others
have similar proofs.
For ease of notation we suppress the dependence
on $L$.
Using Equation \ref{MAINDIFF}, the fact that
the mixed partials commute, and the product rule, we have
\begin{equation}
\label{prelim}
\frac{\partial}{\partial t} \frac{\partial y}{\partial L}=
\frac{\partial y'}{\partial L}=
\frac{\partial (yz)}{\partial L} =
y \frac{\partial z}{\partial L} + z \frac{\partial y}{\partial L}.
\end{equation}
Call this final expression $\Phi$.
Using Equation \ref{prelim} we have
$$
\frac{\partial Y}{\partial t}=
\frac{\partial}{\partial L} \frac{y'}{y}=
\frac{\Phi y-\frac{\partial y}{\partial L}y'}{y^2}=
\frac{\Phi y-\frac{\partial y}{\partial L}yz}{y^2}=
\frac{\Phi-\frac{\partial y}{\partial L}z}{y}=Z.
$$
This gives the formula for $Y'$.
The formulas for the other first derivatives
are similar to this.

Here is how we get the formula for $Z''$.
We first work out that
\begin{equation}
  \label{diffZ}
  z''=-2z+2z^3.
\end{equation}
We then compute
$$Z'' = \frac{\partial z''}{\partial L}=
\frac{\partial(-2z+2z^3)}{\partial L} =
(-2+6z^2)Z.$$



\subsection{The Formula for B}
\label{Matei}

Here is a formula for $B$ in terms of the other quantities.
Matei Coiculescu found this formula and our derivation
follows his ideas.

\begin{equation}
  \label{nice}
B=\frac{x \underline a}{y\underline b} X - \frac{1}{2} Y  - \frac{1}{2y\underline b} Z.
\end{equation}

We will work with
  $a$ and $b$ rather than $\underline a$ and $\underline b$ until the end.
  We have
$$
    (ax-by)'=2x^2-2y^2=2z', \hskip 20 pt a(0)=b(0)=0.
$$
  Integrating, we get
  \begin{equation}
    \label{Matei2}
    ax - by = 2z.
    \end{equation}

Since $x^2+y^2+z^2 \equiv 1$ we have
$  2 x \dot x + 2 y \dot y + 2 z \dot z  =0$.
We also have
$$
  \frac{d}{dt}(x\dot a) = 2x \dot x + ax \dot z, \hskip 30 pt
  \frac{d}{dt}(y\dot b) = 2y \dot y -by  \dot z.
$$
Adding these equations we see that
$$\frac{d(x \dot a + y \dot b)}{dt}=
2x \dot x + 2y \dot y + (ax-by)\dot z =
2x \dot x + 2y \dot y + 2z\dot z = 0.$$
Hence $x \dot a + y \dot a$ is a constant function.
Since $a(0)=b(0)=0$ for all $L$ we have
$\dot a(0)=0$ and $\dot b(0)=0$.  So, the
constant in question is $0$.
Therefore,
     \begin{equation}
      \label{Matei3}
      x\dot a + y \dot b=0.
      \end{equation}

Differentiating Equation \ref{Matei2} with respect to $L$, we have
\begin{equation}
  \label{Matei4}
x \dot a  + a \dot x -y \dot b  - b \dot y=2 \dot z.
\end{equation}  
Subtracting Equation \ref{Matei4} from Equation \ref{Matei3} we get
\begin{equation}
  \label{Matei5}
  2y \dot b - a \dot x  + b \dot y = -2 \dot z.
\end{equation}
Rearranging this, we get
$$
  \dot b = \frac{a\dot x - b \dot y - 2 \dot z}{2y}.
$$
When we make the substitutions
$$
  \underline a=a/2, \hskip 12 pt
  \underline b=b/2, \hskip 12 pt
  X=\dot x/x, \hskip 12 pt
  Y=\dot y/y, \hskip 12 pt
  Z=\dot z, \hskip 12 pt
$$
we get Equation \ref{nice}.


\subsection{Variation of the Z Coordinate}
\label{ODE}

\begin{lemma}
  \label{Wron}
  Let $\pi \sqrt 2<L<M$. Then $z_M=z_L$ at most once on $(0,L)$.
\end{lemma}

\startproof
We already mentioned above that
$z''=-2z+2z^3$.
Let $z_L$ and $z_M$ be two solutions to this differential
equation. Consider the ratio $\phi=z_M/z_L$.
This quantity is positive on $(0,L/2]$.
By L'hopital's rule we can continuously
extend $\phi$ to $0$, and we have $\phi(0)>1$.

We have
\begin{equation}
\label{wron2}
\frac{d\phi}{dt} = \frac{W}{z_L^2}, \hskip 30 pt
W=z_L z_M' - z_M z_L', \hskip 30 pt
\end{equation}
If $z_L \not =0$ then $W$ and $\phi'$ have the same sign.
We compute
\begin{equation}
W'=z_L z_M'' - z_M z_L''=
2z_Lz_M(z_M^2-z_L^2).
\end{equation}

Suppose there is some smallest time $t \in (0,L/2]$ where $z_L(t)=z_M(t)$.
Note that $W' \not = 0$ on $(0,t)$.  Also, $W'>0$ on some small interval
$(0,\epsilon)$ because $z'_M(0)>z'_L(0)$.  Hence
$W'>0$ on $(0,t)$.  Hence $\phi$ is
increasing on $(0,t)$. In particular, $\phi(t)>1$.  Hence $z_M(t)>z_L(t)$, a contradiction.

If there is no time $t \in (L/2,L)$ where $z_M(t)=z_L(t)$,
then we are done.  Otherwise, let
$t_0$ be the smallest such time.
We have $z_L(t_0)=z_M(t_0)<0$.
Since $z_L(t_0-\epsilon)<z_M(t_0-\epsilon)$
for small $\epsilon>0$,
we have $z_M'(t_0) \leq z_L'(t_0)<0$.
Since these two functions are solutions of a
second order ODE, namely Equation \ref{diffZ},
they cannot have the
same initial conditions at $t_0$. Hence
$z_M'(t_0)<z_L'(t_0)<0$.

Let $\zeta_L=-z_L$ and $\zeta_M=-z_M$.  We
consider these functions on the interval
$(t_0,L)$.  These
are solutions of the same differential
equation, with initial conditions
$\zeta_L(t_0)=\zeta_M(t_0)$ and
$0<\zeta_L'(t_0)<\zeta_L'(t_0)$.
The same argument as above, applied to
$\zeta_L$ and $\zeta_M$, shows
$z_L(t)>z_M(t)$ for $t \in (t_0,L]$.
  \endproof

\begin{lemma}[Z variation]
$Z_L$ changes sign
  at most once on $[0,L]$ and $Z_L \geq 0$ on $[0,L/2]$.
\end{lemma}

\startproof
For the first statement, suppose
there are $3$ points $t_1,t_2,t_3$ where
$Z_L(t_i)$ for
$i=1,2,3$ alternates sign.  But then
for $\epsilon$ sufficiently small,
the difference
$z_{L+\epsilon}(t_i)-z_L(t_i)$ also alternates sign
for $i=1,2,3$. This contradicts Lemma \ref{Wron}.
So, there at most one $t_0 \in [0,L]$ where
$Z_L$ changes sign.  The second statment follows
from the analysis in Lemma \ref{Wron}, which
showed that $z_M(t)> z_L(t)$ when $L<M$ and $t \in (0,L/2)$.
\endproof

\subsection{Asymptotics}

If $f$ and $g$ are functions of $L$, we write
$f \sim g$ if $f/g \to 1$ as $L \to \infty$.
In case $g$ is just a constant function, we
will write $f \sim_1 g$ if, additionally,
$\dot f \sim 0$. Given that we are working
with analytic functions it is not surprising
that whenever $f \sim {\rm const.\/}$ we also
have $\dot f \sim 0$.  However, we don't
know {\it a priori\/} that our functions
have analytic continuations at $\infty$,
so we have to explicitly deal with their
derivatives.
In this section we prove the following results.
$$
  Y_L(L/2)=X_L(L) \sim_1 0, \hskip 20 pt
  X_L(L/2)=Y_L(L) \sim_1 -1/2,
  $$
\begin{equation}
  \label{asy1}
  Z_L(L) \sim_1 -1, \hskip 20 pt
  B_L(L) \sim_1 1/2, \hskip 20 pt Z_L'(L) \sim_1 0.
\end{equation}
These various features are already apparent in Figure 7.1.
Here we have written e.g. $X_L$ in place of $X$ to explicitly
indicate how the quantity depends on $L$.  That is,
$X_L = \dot x_L/x_L$, where $x_L$ is the solution to the
ODE with initial conditions associated to $L$.

Our first two results reduce the number of different quantities
we have to deal with.

\begin{lemma}
  \label{yequal}
  $Y_L(0)=Y_L(L)$.
\end{lemma}

\startproof
Since $(\log(y))'=z$,
$$\log y(L)=\log y(0) +\int_0^L z(s)ds.$$
Therefore
\begin{equation}
  \label{integrate00}
  Y_L(L)-Y_L(0)=\lim_{\epsilon \to 0} \frac{I_{L,L+\epsilon}-I_{L,L}}{\epsilon},
  \hskip 30 pt I_{L,L+\epsilon}=\int_0^L z_{L+\epsilon} (s)ds.
\end{equation}
Note that $I_{L,L}=0$ and
\begin{equation}
  |I_{L,L+\epsilon}| = |I_{\epsilon,L_{\epsilon}}| = \bigg|\int_0^{\epsilon} z_{L+\epsilon}(t)\ dt\bigg| \leq \epsilon^2.
\end{equation}
The last equation comes from the fact that $|z'| \leq 1$, which forces $|z(t)| \leq \epsilon$ on
$[0,\epsilon]$.
The limit in Equation \ref{integrate00} is therefore $0$.
Hence $X_L(0)=X_L(L)$.
\endproof

\begin{lemma}
  \label{yequal2}
  $X_L(L/2)=Y_L(0)$.
\end{lemma}

\startproof
We have the relations
$$x_L(L/2)=y_L(0), \hskip 30 pt
x_{L+\epsilon}(L/2)=y_{L+\epsilon}(\epsilon/2)=y_{L+\epsilon}(0) + O(\epsilon^2).
$$
The last equality comes from the fact that the function
$t \to y_{L+\epsilon}(t)$ has its local minimum at $0$.
From these relations we have
$$\dot x_L(L/2)=\lim_{\epsilon \to 0} \frac{x_{L+\epsilon}(L/2)-x_L(L/2)}{\epsilon}= 
\lim_{\epsilon \to 0} \frac{y_{L+\epsilon}(0) + O(\epsilon^2)-y_L(0)}{\epsilon}=\dot y_L(0).$$
The lemma follows from this last equation and from $x_L(L/2)=y_L(0)$.
\endproof


\begin{lemma}
  \label{asymptote1}
  $Y_L(0) \sim_1 -1/2$
\end{lemma}

\startproof
We set $y=y_L(0)$.
By the Inverse Function Theorem we have
\begin{equation}
  Y_L(0)=\frac{1}{y \times \frac{\partial L}{\partial y}(y)}.
  \end{equation}
Using Equation \ref{periodXX} we can get an explicit formula for $L$ in terms of $y$.
Define
\begin{equation}
  f(y)=\frac{1}{\sqrt{1+2y \sqrt{1-y^2}}} \hskip 15 pt
  g(y)=\frac{1-2y \sqrt{1-y^2}}{1+2y \sqrt{1-y^2}}.
\end{equation}
In Equation \ref{periodXX}, we have  $\alpha^2=y \sqrt{1-y^2}$.
Therefore, by Equation \ref{periodXX},
\begin{equation}
  L(y)=4f(y){\cal K\/} \circ g(y)
\end{equation}
We compute this in Mathematica, and we get a polynomial expression
terms of $\sqrt y$ and $K={\cal K\/} \circ g(y)$ and $E={\cal E\/} \circ g(y)$.  Taking the
series expansions of the coefficients, we find that
\begin{equation}
  \label{ASY1}
  Y_L(0) = \frac{-1-5y+ \cdots}{\Delta}, \hskip 15 pt
  \Delta = (2+ 12 y+\cdots) E + (-4y - 24 y^2 + \cdots) K.
    \end{equation}
Given that $g(y) \sim 1-4y$, we see from Equations \ref{ASY} and
\ref{ASY1} that
$Y_L(0) \sim -1/2$.
Similarly
  \begin{equation}
    \frac{\partial}{\partial y} Y_L(0) = \frac{(48y +  \cdots)E + (-48 y + \cdots)K}{\Delta^2} \sim 0.
  \end{equation}
  Since $dy/dL \sim 0$ we have {\it a fortiori\/} that $\frac{d}{dL}Y_L(0) \sim 0$.
  \endproof


\begin{lemma}
  $X_L(0) \sim_1 0$.
\end{lemma}

\startproof
We differentiate 
$x^2+y^2+z^2=1$ and use $z_L(0)=0$ to get
\begin{equation}
\label{sumsquare}
x_L^2(0)X_L(0) + y_L^2(0)Y_L(0)=0.
\end{equation}
We see that $X_L(0) \sim 0$ because
$x_L(0) \sim 1$ and
$y_L(0) \sim 0$ and $Y_L(0) \sim -1/2$ (a finite number).
Differentiating Equation \ref{sumsquare} with respect to $L$ and
using the product rule we see that   $\frac{d}{dL} X_L(0) \sim 0$.
\endproof


  \begin{lemma}
    \label{Zasy}
    $Z_L(L) \sim -1$.
    \end{lemma}

  \startproof
Let $M=L+\epsilon$.  Let
$g_L$ and $g_M$ respectively denote
the flowlines in the loop level set of
periods $L$ and $M$ respectively that
start at the points
$(x_L(0),y_L(0),0)$ and
$(x_M(0),y_M(0),0)$ and travel for time $L$.
We have $z_L(L)=0$ because $g_L$ is a
perfect flowline.

We can write $\gamma_M=g_M|h_M$  where
$\gamma_M$ is the perfect flowline and
$h_M$ is the flowline which starts at
$(x_M(0),y_M(0),0)$ and travels for time $\epsilon$.
By Equation \ref{additive}, we have
$$
-Z_L(L) = \lim_{\epsilon \to 0} \frac{z_{L+\epsilon}(\epsilon)}{\epsilon}=
  \lim_{\epsilon \to 0} \frac{z_{L+\epsilon}(\epsilon)-z_L(\epsilon)}{\epsilon}
  +\lim_{\epsilon \to 0}\frac{z_{L}(\epsilon)}{\epsilon}.
$$
  We have
  $$z_M(\epsilon) = (1 - 2y_M^2(0)) \epsilon + O(\epsilon^2),$$ for
  any $M$.
  This gives us the formula
$$
    Z_L(L)=\frac{d}{dL}(1-2 y_L(0)^2) - 1+2 y_L(0)^2 =$$
    \begin{equation}
\label{formulaZ}
-2 y_L(0) \frac{d}{dL} y_L(0) - 1 + 2y_L^2(0)=
     -2y_L^2(0) Y_L(0) -1 + 2y_L^2(0).
\end{equation} 
   Since $Y_L(0) \sim -1/2$ and $y_L(0) \sim 0$, Equation \ref{formulaZ}
tells that $Z_L(L) \sim -1$.
    Differentiating the rightmost expression in
    Equation \ref{formulaZ} with respect to $L$, and using
the product rule, we see that
    $\frac{d}{dL} Z_L(L) \sim 0$.
    \endproof

The rest of the relations for $X_L$ and $Y_L$
follow from the ones we have established above,
from Lemmas \ref{yequal} and \ref{yequal2}, and
the fact that $X_L+Y_L$ is a constant function.

\begin{lemma}
  $Z'_L(L) \sim_1 0$.
\end{lemma}

\startproof
Since $z_L(L)=0$ we have 
\begin{equation}
\label{diffZprime}
Z'_L(L)=-4y_L^2(L) Y_L(L).
\end{equation}
But $y_L(L) \sim 0$ and $Y_L(L) \sim -1/2$.
This gives $Z'_L(L) \sim 0$.
The calculation in Lemma \ref{asymptote1}
shows also that $\frac{d}{dL} y_L(L)=0$
because (in the notation of Lemma \ref{asymptote1})
we have $y_L(L)=y_L(0)=y$.
Differentiating Equation \ref{diffZprime} with
respect to $L$ and using the product rule,
as above, we see that $\frac{d}{dL}Z'_L \sim 0$.
\endproof

\begin{lemma}
  $\frac{d}{dL}(x_L(L) a_L(L)) \sim 0$.
\end{lemma}

\startproof
From the proof of 
Lemma \ref{ABOUND},
we see that
\begin{equation}
  x_L(L)a_L(L)=2 z_L(L/4) + 2\phi_L, \hskip 20 pt
  \phi_L =\int_0^{L/4} y_L^2\ dt.
\end{equation}
We deal with these terms one at a time.
Referring to Equation \ref{periodXX} we have
$z_L(L/4)=\sqrt{1-2\alpha_L^2}$.
Here $\alpha_L \sim 0$.
This leads to  $\frac{d}{d\alpha}(Z_L(L/4)) \sim 0$.
A calculation like the one done in
Lemma \ref{asymptote1} shows that $|dL_{\alpha}/d\alpha| \sim \infty$.
Hence $d\alpha_L/dL \sim 0$.  But then, by the
chain rule, $\frac{d}{dL}z_L(L/4) \sim 0$.

We have
\begin{equation}
  \frac{d\phi_L}{dL}=\int_0^{L/4} \frac{\partial}{\partial L} (y_L)^2\ dt + \frac{1}{4}y_L(L/4).
\end{equation}
Referring to Equation \ref{periodXX} we have
$y_L(L/4)=\alpha$.  So, the same argument as for $Z_L(L/4)$ now shows that
$\frac{d}{dL} y_L(L/4) \sim 0$.
Finally, we have
$$\int_0^{L/4} \frac{\partial}{\partial L} (y_L)^2\ dt=
2\int_0^{L/4} y_L^2 \dot Y_L\ dt \leq 2\max_{[0,L/4]} |Y_L| \times \int_0^{L/4} y_L^2.$$
From the proof of Lemma \ref{ABOUND} we know that the last integral
converges to $0$ as $L \to \infty$.  So, to finish the proof we just
have to show that $Y_L$ is uniformly bounded on $[0,L/4]$.
Since $Y_L'=Z_L$, the Z Variation Lemma tells us that
$Y_L$ is monotone increasing on $[0,L/2]$.  But $Y_L(0) \sim 0$ and $Y_L(L/2) \sim 1/2$.
Hence $\max_{[0,L/4]} |Y_L|<1$ for $L$ large.
\endproof

\begin{lemma}
  \label{asymptote2}
  $B_L(L) \sim_1 1/2$.
\end{lemma}

\startproof
By the Reciprocity Lemma and the Asymptotic Theorem, we have
$$x_L(L) \underline a_L(L)=y_L(L) \underline b_L(L) \sim 2.$$
Hence
$$B_L(L)=X_L(L) - \frac{1}{2} Y_L(L)  - \frac{1}{y_L(L)\underline b_L(L)} Z_L(L) \sim$$
\begin{equation}
  \label{nice3}
  X_L(L) - \frac{1}{2} Y_L(L)  - \frac{1}{4} Z_L(L) \sim
  0  + (-1/2)(-1/2)  + (-1/4) (-1) =1/2.
  \end{equation}
Since $b_L(L) \sim \infty$ and $B_L(L) \sim 1/2$, we
see that $\frac{d}{dL} b_L(L) \sim 0$.
We also already know that $df/dL \sim 0$ for $f(L)$ equal to any of the following:
$$X_L(L), Y_L(L), Z_L(L), y_L(L)\underline b_L(L).$$
Also, we know that $y_L(L) \underline b_L(L) \sim 2.$
Using all this information, and the product and quotient rules for
differentiation, we see that  $\frac{d}{dL} B_L(L)=0$.
\endproof

\subsection{Variation of the Y Coordinate}

The purpose of this section is to prove the following result.

\begin{lemma}[Y Variation]
Let $\delta_0=1/7$.
  \label{yvanish}
  If $L$ is sufficiently large then:
  \begin{enumerate}
\item $|Y_L|,|Z_L|<5$ on $[L-1,L]$.
  \item $Y_L(L)<-\delta_0$.
  \item $Y_L'<-\delta_0$ on $[L-1,L]$.
  \item $Y_L(L-1)>\delta_0$.
  \item $Y_L>0$ on $(L/2,L-1]$.
\end{enumerate}
\end{lemma}

\noindent
{\bf Proof of Statement 1:\/}
Let $\phi_L(t)=-Z_L(L-1)$.  This function satisfies the
differential equation
$$
  \phi_L(0)=-Z_L(L) \sim 1, \hskip 15 pt
  \phi'_L(0)=Z_L'(L) \sim 0, \hskip 15 pt
  \phi_L''(t)=(-2 + 6 z_L^2(t)) \phi_L(t).
$$
For the last equality we used the fact that $z_L^2(L-t)=z_L^2(t)$.
The solutions to this equation converge in the $C^{\infty}$ sense to
the solutions of the equation
\begin{equation}
  \phi(0)=1, \hskip 30 pt
  \phi'(0)=0, \hskip 30 pt
  \phi''=(-2 + 6 z^2) \phi.
  \end{equation}
Here $z$ satisfies $z''=-2z+2z^3$ with initial conditions $z(0)=0$ and $z'(0)=1$.
Since $\phi'' \in [-2,4] \phi$, and since $\cos(t \sqrt 2)>0$ on $(0,1]$, we have
\begin{equation}
\cos(t \sqrt 2) \leq \phi(t) \leq \cosh(2t).
\end{equation}
Since $\phi_L \to \phi$ we see that $|\phi_L|<2$ once $L$ is large.
Hence $|Z_L|<4$ on $[L-1,1]$.  Since $Y_L(L) \sim -1/2$ we have
$|Y_L|<5$ on $[L-1,L]$. \endproof
\newline
\newline
{\bf Proof of Statement 2:\/} This follows from the fact that $Y_L(L) \sim -1/2$.
    \newline \newline
{\bf Proof of Statement 3:\/}
Let $\phi_L$ and $\phi$ be the functions from the previous lemma.
For $t \in [0,1]$ we have (because $\phi$ is monotone decreasing)
$$
Y'_L(L-t)=Z_L(L-t)=-\phi_L(t)<\epsilon - \phi(t) \leq $$
\begin{equation} 
  \epsilon - \phi(1)  \leq
\epsilon - \cos(\sqrt 2) < -1/7
\end{equation}
once $\epsilon$ is sufficiently small.  We can arrange
this by taking $L$ sufficiently large. \endproof
\newline
\newline
{\bf Proof Statement 4:\/}
To estimate $Y_L(L-1)$ we note that
$$
Y_L(L-1) = Y_L(L) - \int_{L-1}^L Z_L\ dt =
Y_L(L) + \int_0^1 \phi_L\ dt > $$
\begin{equation}
- \epsilon -1/2 + \int_0^1 \phi\ dt=
-\epsilon  -1/2 + \frac{\sin(\sqrt 2)}{\sqrt 2}>1/7,
\end{equation}
once $\epsilon$ is sufficiently small. \endproof
\newline
\newline
{\bf Proof Statement 5:\/} Suppose this is false.
Since $Y_L(L/2) \geq 0$ and
$Y_L'(L/2)=Z_L(L/2)>0$ we see that
$Y_L$ is somewhere positive on $(L/2,L-1]$.
Also, $Y_L(L-1)>0$ and $Y_L(L)<0$.
If $Y_L=0$ somewhere else on $(L/2,L-1]$ then
  $Y_L$ switches signs at least $3$ times.
  But then $Z_L=Y_L'$ switches sign at least
  twice. This contradicts the Z Variation Corollary.
  \endproof

  \subsection{Variation of the B Coordinate}

\begin{lemma}[B variation]
  \label{close}
As $L \to \infty$, the function $Y_L+B_L$
converges to $0$ in the $C^1$ sense.
\end{lemma}

\startproof
We sometimes suppress the dependence on $L$ in our notation.
By Equation \ref{asy1} we have $|Y(L)+B(L)|<\epsilon/2$ if
$L$ is sufficiently large.  To finish the proof, it suffices to
show that $|B'+Y'|<\epsilon/2$ on $[L-1,1]$ for large $L$.
Combining our derivative formulas with the
preceding two results, we have
$$
|B'+Y'| \leq
\bigg|\frac{y}{\underline b}\bigg|\bigg(\max_{[L-1,L]} |Y|+|B|\bigg)
\leq 
\frac{10 y}{b}<10 y.$$
  For the last inequality, we note that $b(L/2)>1$ when $L$ is large and
  $b'>0$ on $[L/2,L]$.  Hence $b>1$ on $[L-1,1]$.
  As $L \to \infty$ the maximum value of $y$ on $[L-1,L]$ tends to $0$.
  \endproof



  \subsection{The Vanishing Point}

  In this section we prove the first half of the
  Monotoniticy Theorem.  That is, we show that
  $\underline{\dot b_L}$ vanishes
    exactly once on $(L/2,L)$.  This is the same
  saying that $B_L$ vanishes exactly once on
  $(L/2,L)$.  Here is the crucial step.
  
\begin{lemma}
  $B_L$ vanishes exactly once in $(L-1,L]$, and $B_L(L-1)<0$.
\end{lemma}

\startproof
Combining the Y Variation Lemma and the B Variation Lemma,
we get that $B_L(L-1)<0$ and $B_L(L)>0$ and $\dot B_L>0$ on $[L-1,L]$.
\endproof

    Let $t_1 \in [L/2,L-1]$ be the smallest value such that
    $Z \leq 0$ on $[t_1,L-1]$.
    
    \begin{lemma}
      $B_L<0$ on $[t_1,L-1]$.
    \end{lemma}

    \startproof
    Since $Z_L(L-1)<0$ we know that $t_1 \in [L/2,L-1)$.
    We introduce the function
    $\phi(t)=-B_L(L-1-t)$.
    We have $\phi(0)>0$ and
    $\phi'(t)=B_L'(L-1-t)$.
Hence
$$\frac{\partial \phi}{\partial t}=\frac{y_L(L-1-t)}{\underline b_L(L-1-t)} \times \bigg(Y_L(L-1-t) + \phi(t)\bigg) - 2 Z_L(L-1-t).$$
By the Y Variation Lemma and the definition of $t_1$ we have
$\phi'=\mu_1 \phi + \mu_2$
where $\mu_1$ and $\mu_2$ are non-negative functions on $[0,L-1-t_1]$.
Since $\phi(0)>0$ we have $\phi>0$ on $[0,L-1-t_1]$.
Hence $B_L<0$ on $[t_1,L-1]$.
\endproof

If $t_1=L/2$ this next lemma is vacuous.

\begin{lemma}
  $B_L<0$ on $(L/2,t_1)$.
  \end{lemma}

\startproof
This follows from Equation \ref{nice} and these inequalities on $[L/2,t_1)$:
\begin{itemize}
\item The quantities $x_L,y_L,\underline a_L,\underline a_L$ are all positive.
\item Since $X_L(L/2) \leq 0$ and $X_L'=-Z_L \leq 0$ on $(L/2,t_1)$, we have $X_L \leq 0$.
\item By the Y Variation Lemma, $Y_L>0$.
\item Since $Z_L$ changes sign only at $t_1$, and
  $Z_L(L)<0)$, we have  $Z_L \geq 0$.
\end{itemize}
This completes the proof.
\endproof



At this point we have established the fact that
there is a unique value $t_L \in (L-1,L)$
where $\underline{\dot b_L}$ vanishes.
It only remains to show that the function
$L \to t_L$ is monotone increasing.  Let
\begin{equation}
  \beta_L(s)=B_L(L-s).
\end{equation}
The domain for all these functions is $[0,1]$.
There is a unique $s_L \in (0,1)$ such that
$\beta_L(s_L)=0$. In fact, $t_L=L-s_L$.
Below we will show that $ds_L/dL \sim 0$, which implies that
$dt_L/dL \sim 1$.  This does it.

  \subsection{Variation of Some Auxiliary Quantities}

  We start with a
  preliminary result.
  
  \begin{lemma}
    $\max_{[0,1]}|Z| \sim 0$.
  \end{lemma}

  \startproof
    We have $Z(0)\sim 0$ and
    $|Z''| \leq 4|Z]$.  Since $Z>0$ on $(0,1]$,
    the same kind of comparison argument used in
    the proof of the Y Variation Lemma now shows that
    $\max_{[0,1]} |Z| \leq Z(0) \cosh(2) \sim 0$.
    \endproof

    Now we study how various quantities associated to the
    differential equation for $\beta$, given below, vary with $L$.
    To simplify our  notation we will write $f$ in place of $f_L$.  Define

  \begin{equation}
  \delta(t)=\frac{y(L-t)}{\underline b(L-t)}, \hskip 30 pt
  \phi(t)=Y(L-s), \hskip 30 pt
  \psi(t)=Z(L-s).
  \end{equation}


  \begin{lemma}[Auxiliary Variation]
    For each choice $f=\delta, \phi, \psi$, we have $\max_{[0,1}] |\dot f| \sim 0$.
  \end{lemma}

  \startproof
  We treat the functions one at time.
  Consider $f=\delta$.
  Using the product rule and the definitions of $B$ and $Y$ we see that
  $$\frac{\partial \delta}{\partial L}(t)= \frac{y(L-t)}{\underline b(L-t)} (Y(L-t)-B(L-t)).
  $$
  By the Y Variation Lemma, we have $|Y|<100$ on $[L-1,L]$.
  By the B Variation Lemma, we have $|B|<101$ on $[L-1,L]$
  for $L$ sufficiently large.  At the same time
  $|\underline b| \geq 1$ on $[L-1,L]$ for $L$ sufficiently
  large and $\max_{[L-1,L]} |y| \sim 0$.
  Putting together all these ingredients gives the result.
  \newline

  Consider $f=\psi$, and define
   $\eta=\partial \psi/\partial L$.
 From the differential equation for $Z''$ and the fact that
 $z_{L-t}=z_t$ we get
 $$\psi''(t) = (-2 + 6z^2(t)) \psi.$$
 Differentiating with respect to $L$ and using the fact that
 the mixed partials commute, we see that
 $$\eta''(t) = (-2+6 z^2(t) \eta(t) + 12 Z(t)z^2(t)\psi(t).$$
 From the Y Variation Lemma and from Statement 1 we now see that
 \begin{equation}
   |\eta''| \leq 4 |\eta(t)| + \epsilon,
 \end{equation}
 where $\epsilon \sim 0$.
 Given our asymptotics, we also have
 $\eta(0) \sim 0$ and
 $\eta'(0) \sim 0$.
 The same kind of comparison argument as above
 gives us the desired result.
 \newline

 Consider $f=\phi$ and let
 $\mu=\partial \phi/\partial L$
 and let $\eta$ be as in the previous lemma.
 We have $\phi'=-\psi$.  Differentiating with
 respect to $L$ we get $\mu'=-\eta$.
 As the same time our asymptotics tell us that
 $\mu'(0) \sim 0$.  The bound on $|\eta|$ now
 gives us the bound on $|\mu|$.
 \endproof

 \subsection{The End of the Proof}

 We return to the function $\beta(t)=B(L-t)$.
 The function
$\beta$ satisfies the differential equation:
\begin{equation}
\beta'(t)=\delta(t)(\phi(t)-\beta(t)) - \psi(t).
\end{equation}
Differentiating with respect to $L$, we find that
$$(\dot \beta)' = \dot \delta(\phi-\beta) +\delta(\dot \phi - \dot \beta) - \dot \psi.$$
Given the Y Variation Lemma and the B Variation Lemma, we see that
\begin{equation}
  |\dot \beta'| \leq \epsilon_1 \dot \beta + \epsilon_2
\end{equation}
where $\epsilon_1, \epsilon_2 \sim 0$.
We also have the initial condition
$\dot \beta(0) \sim 0$.
A standard comparison argument shows that
$\max_{[0,1]} |\dot \beta| \sim 0$.

By definition
\begin{equation}
  \beta_L(s_L)=0.
\end{equation}
Using implicit differentiation, we see that
\begin{equation}
  \dot s_L = -\frac{\dot \beta}{\beta'}.
\end{equation}
By the Y Variation Lemma and the B Variation Lemma together,
we have $\max_{[0,1]}|\beta'_L|>1/8$ for large $L$.
But but then we see that $\dot s_L \sim 0$.

Our proof of the Monotonicity Lemma is done.

\newpage


